Physics-Informed Feature Engineering 1D-CNN for Multilayer Cloud Detection from Geostationary Satellites

Multilayer cloud detection from active--passive observation is vital for numerical weather prediction. In this study, channel selections derived from threshold-based algorithms are embedded as feature-engineering priors into a 1D-CNN, and machine learning (ML) is used to learn latent physical relationships to simplify physical retrievals for operational deployment. The results show that the 1D-CNN achieves a multilayer-cloud probability of detection ($\mathrm{POD}{\mathrm{mul}}$) of 0.620 and a false alarm rate ($\mathrm{FAR}{\mathrm{mul}}$) of 0.240, outperforming the conventional threshold algorithm ($\mathrm{POD}{\mathrm{mul}} = 0.558$, $\mathrm{FAR}{\mathrm{mul}} = 0.369$). These results demonstrate that prior physical knowledge derived from radiative transfer theory can serve as an effective feature-engineering prior. Further experiments show that ML-revealed physical mechanisms can also enhance traditional algorithms. Replacing AGRI channel 12 (C12, centered at $10.8~\mu\mathrm{m}$) with channel 13 (C13, centered at $12.0~\mu\mathrm{m}$) increased $\mathrm{POD}{\mathrm{mul}}$ from 0.558 to 0.609 without materially affecting $\mathrm{FAR}{\mathrm{mul}}$. However, for AHI, substituting the $11.2~\mu\mathrm{m}$ channel with the $12.3~\mu\mathrm{m}$ channel yielded negligible improvement. In addition to spectral response function (SRF) mismatches, a primary contributing factor is the channels' on-orbit radiometric stability. Hence, physics-informed machine-learning methods appear promising for advancing remote-sensing AI, while sensor-specific characteristics must be considered during operational transfer.

==> rev_pack.tex <==
% rev_pack.tex  ——  公共配置文件，正文和回复信都要 \input 它
\usepackage{lineno}        % 行号（方便审稿人定位）
\usepackage{soul}          % 高亮修改内容
\usepackage{xcolor}        % 颜色支持
\usepackage{tcolorbox}      % 回复信里的评论框/引用框
\tcbuselibrary{skins, breakable}

% ===== 1. 修改高亮开关（一键切换是否显示高亮）=====
\newif\ifshowrev
\showrevtrue   % 显示高亮；最终稿改为 \showrevfalse 即可隐藏

% 正文修改高亮命令：\highlight{新内容}   —— 蓝色斜体
\colorlet{revcolor}{blue}   % 颜色定义为蓝色（可改为 blue!80!black 等）
\ifshowrev
  \newcommand{\highlight}[1]{\textcolor{revcolor}{\itshape #1}}   % 斜体，不加粗
\else
  \newcommand{\highlight}[1]{#1}
\fi

% ===== 2. 回复信专用样式 =====
% 审稿人评论框
\newtcolorbox{reviewercomment}{
  colback=gray!10,    % 极淡的灰色背景
    colframe=gray!40,   % 浅灰色的边框
    boxrule=0.5pt,      % 边框粗细
    arc=3pt,            % 圆角
    left=4pt, right=4pt, top=4pt, bottom=4pt, % 内边距
    fontupper=\small    % 审稿人意见字体稍微缩小一点，更易区分
}

% 正文修改引用框（和正文联动）
\newtcolorbox{revquotebox}{
  colback=gray!5, 
  colframe=gray!70,
  boxrule=0.5pt, 
  arc=2pt,
  title=Modified in Manuscript, 
  fonttitle=\bfseries,
  coltitle=blue,  
  fontupper=\color{blue}\itshape,   % 框内正文：蓝色 + 斜体
  breakable
}

\newcommand{\revhead}[3]{%
  \par\noindent\textbf{#1} (Page #2, #3):\par
}
% ==============================================================================
% 第二部分：你的所有修改片段！！！全部放这里！！！
% 以后只改这里！！！
% ==============================================================================
% 审稿人 1 意见 1
\newcommand{\RevAComAChaA}{Physics-Informed Feature Engineering 1D-CNN for Multilayer Cloud Detection from Geostationary Satellites}%

\newcommand{\RevAComAChaB}{To address these limitations, recent studies have resorted to physics-informed feature engineering with promising results~\cite{li_physics-driven_2024}. To further probe the interplay between physics-informed feature engineering and machine learning, three complementary lines of investigation were undertaken in this work:}%

\newcommand{\RevAComAChaC}{ Embedding physical priors to guide feature engineering (via threshold-derived channel selections) reduces complexity and improves interpretability—solving the trade-off between ML accuracy and operational feasibility.}

% 审稿人 1 意见 2
\newcommand{\RevAComBChaA}{To address ambiguous physical relationships in multilayer cloud radiative transfer, our core innovation physics informed feature engineering leverages 1D-CNNs to extract high dimensional latent features from multi spectral data under physical constraints, overcoming the poor feature representation inherent in threshold-based methods.}

% 审稿人 1 意见 3
\newcommand{\RevAComCChaA}{The proposed network architecture contains approximately 116k trainable parameters. On the AGRI L1 dataset, it achieves an inference time of about 242 seconds and a memory usage of roughly 10.4 MB.
}

% 审稿人 1 意见 4
\newcommand{\RevAComDChaA}{
Specifically, we provide a multilayer cloud detection algorithm for nighttime scenes, denoted CNN\--night, along with detailed evaluation results over different underlying surfaces for the CNN\--SWIR2TIR configuration, as shown in Fig. S1.
}



%审稿人 2 意见 1
\newcommand{\RevBComAChaA}{
Thereby demonstrating that prior physical knowledge derived from radiative transfer theory can serve as a feature engineering prior.
}

%审稿人 2 意见 2
\newcommand{\RevBComBChaA}{
In recent years, pure data-driven deep learning methods have achieved significant progress in cloud detection. For instance, Hu et al. (2021)~\cite{hu2021cdunet} proposed CDUNet, which optimizes cloud boundaries and thin cloud localization using high-frequency feature extraction, multi-scale convolution, and a spatial prior self-attention mechanism. Ma et al. (2023)~\cite{ma2023cnn} designed CNN-TransNet with a dual-branch CNN-Transformer encoder and a differential feature enhancement module, reducing missed detections of thin clouds and false alarms over bright surfaces (e.g., snow, ice, and urban areas).
}
%审稿人 2 意见 3
\newcommand{\RevBComCChaA}{
 However, these methods generally lack physical interpretability. To overcome this limitation, physics-informed deep learning methods incorporate radiative transfer physical laws or prior knowledge into the model. Heidinger et al. (2012)~\cite{heidinger2012naive} trained a naive Bayesian cloud detection scheme based on CALIPSO lidar data, establishing classifiers for different surface types and achieving good performance over both ocean and land. Li et al. (2024)~\cite{li2024physics} used clear\--sky brightness temperatures simulated by a radiative transfer model as prior information and designed a CNN\_TL model with transfer learning to simultaneously retrieve the properties of upper ice clouds and lower water clouds in multilayer clouds from Himawari\--8 passive imager observations. The retrieved cloud top heights showed strong agreement with active sensor products, outperforming the official products. These studies indicate that the cloud detection field is evolving from a pure data-driven paradigm toward a physics-data dual-driven paradigm.
}

%审稿人 2 意见 5
\newcommand{\RevBComEChaA}{
Temporal matching was constrained to a ±5‑minute window between the imager scan time and the active sensor overpass, balancing temporal mismatch with sufficient data retention. Spatial collocation was performed using a nearest‑neighbor matching strategy: for each imager pixel, the closest overlapping footprint from the CPR‑CALIOP product was selected. When multiple active sensor footprints fell within a single imager pixel, the lidar observations were aggregated by taking the mean for continuous variables or the mode for categorical variables to establish a one‑to‑one correspondence.
}

%审稿人 2 意见 11
\newcommand{\RevBComKChaA}{
This study developed a framework that employs prior physical knowledge to guide feature engineering, combined with a 1D‑CNN for feature extraction, for multilayer cloud detection using geostationary imagers such as FY‑4A/AGRI and Himawari‑8/AHI.
}
\newcommand{\RevBComKChaB}{
In future work, this physics–machine learning synergy will be extended to longer time periods and global-scale studies to further validate the proposed paradigm across diverse seasons, surface types, and viewing geometries.
}

